Algorithms for Computing Abelian Periods of Words

Constantinescu and Ilie (Bulletin EATCS 89, 167--170, 2006) introduced the notion of an \emph{Abelian period} of a word. A word of length $n$ over an alphabet of size $\sigma$ can have $\Theta(n^{2})$ distinct Abelian periods. The Brute-Force algorithm computes all the Abelian periods of a word in time $O(n^2 \times \sigma)$ using $O(n \times \sigma)$ space. We present an off-line algorithm based on a $\sel$ function having the same worst-case theoretical complexity as the Brute-Force one, but outperforming it in practice. We then present on-line algorithms that also enable to compute all the Abelian periods of all the prefixes of $w$.

==> algo_online_array.tex <==
\begin{algo}[eqtab]{AbelianPeriod-array}{w,n}
\SET{T[0,1]}{1}
\label{algo2-line1}
\DOFORI{i}{2}{n}
  \DOFORI{p}{1}{i-1}
\label{algo2-line2}
    \DOFORI{h}{0}{\mbox{min}\{p-1,i-p-1\}}
	\IF{T[h,p]=i-1}
	  \SET{d}{(i-h)\bmod p}
	  \IF{d\ne 0}
		\IF{\PVW(i-d+1,d)\subset\PVW(i-d-p+1,p)}
			\SET{T[h,p]}{i}
		\FI
	  \ELSE
		\IF{\PVW(i-p+1,p)=\PVW(i-2\times p+1,p)}
			\SET{T[h,p]}{i}
		\FI
	  \FI
	\FI
    \OD
  \OD
  \DOFORI{h}{0}{\lfloor i/2\rfloor-1}
    \IF{\PVW(1,h)\subset\PVW(h+1,i-h)}
      \SET{T[h,i-h]}{i}
    \ELSE
      \SET{T[h,i-h]}{-1}
    \FI
  \OD
\OD
\RETURN T
\end{algo}

